Type safety of rewrite rules in dependent types

The expressiveness of dependent type theory can be extended by identifying types modulo some additional computation rules. But, for preserving the decidability of type-checking or the logical consistency of the system, one must make sure that those user-defined rewriting rules preserve typing. In this paper, we give a new method to check that property using Knuth-Bendix completion.

==> macros.tex <==
% proof trees
\newenvironment{ded}
   {\begin{center}\begin{prooftree}}
   {\end{prooftree}\end{center}}
\newcommand\pra[3][]{\[#2\justifies #3\using\mbox{(#1)}\]}
\newcommand\prb[4][]{\[#2\quad #3\justifies #4\using\mbox{(#1)}\]}
\newcommand\prc[5][]{\[#2\quad #3\quad #4\justifies #5\using\mbox{(#1)}\]}
%\newcommand\qed[2][]{\justifies #2\using\mbox{(#1)}}

% biblios
\newcommand\shortbib{short,abbrev,short-names,mybib}
\newcommand\longbib{long,abbrev,long-names,mybib}

% miscellaneous
\newcommand\hide[1]{}
\renewcommand\show[1]{#1}
\newcommand\bu{$\bullet$}
\newcommand\hsp[1][3ex]{\hspace*{#1}}
\newcommand\vsp[1][1mm]{\vspace*{#1}}
\newcommand\moins{\setminus}
\newcommand\vide{\emptyset}
\newcommand\eg{{\em e.g.} }
\newcommand\ie{{\em i.e.} }
\newcommand\etal{{\em et al} }
\newcommand\ala{{\em \`a la} }
\newcommand\furl[1]{\footnote{\url{http://#1}}}

% substitutions
\newcommand\xt{\{x\to t\}}
\newcommand\xu{\{x\to u\}}
\newcommand\xv{\{x\to v\}}
\newcommand\yu{\{y\to u\}}
\newcommand\yv{\{y\to v\}}
\newcommand\yw{\{y\to w\}}
\newcommand\xup{\{x\to u'\}}
\newcommand\XU{\{X\to U\}}
\newcommand\XS{\{X\to S\}}
\newcommand\xS{\{x\to S\}}

% vectorial substitutions
\newcommand\vyu{\{\vy\to\vu\}}
\newcommand\vyt{\{\vy\to\vt\}}
\newcommand\vxt{\{\vx\to\vt\}}
\newcommand\vxtp{\{\vx\to\vt'\}}
\newcommand\vxl{\{\vx\to\vl\}}
\newcommand\vxv{\{\vx\to\vv\}}
\newcommand\vxS{\{\vx\to\vS\}}
\newcommand\vxu{\{\vx\to\vu\}}
\newcommand\vxup{\{\vx\to\vu'\}}
\newcommand\vzv{\{\vz\to\vv\}}

% function names
\newcommand\lfp{\mr{lfp}}
\newcommand\glb{\mr{glb}}
\newcommand\lub{\mr{lub}}
\newcommand\dom{\mr{dom}}
\newcommand\codom{\mr{codom}}
\newcommand\FV{\mr{FV}}
\newcommand\Var{\mr{Var}}
\newcommand\Pos{\mr{Pos}}
\newcommand\lex{\mr{lex}}
\newcommand\mul{\mr{mul}}
\renewcommand\prod{\mr{prod}}
\newcommand\stat{\mr{stat}}

% arrows
\renewcommand\a{\rightarrow}
\newcommand\A{\Rightarrow}
\renewcommand\aa{\leftrightarrow}
\renewcommand\AA{\Leftrightarrow}
\newcommand\la{\leftarrow}
\newcommand\lA{\Leftarrow}
\newcommand\ad{\downarrow}
\newcommand\Ad{\Downarrow}
\newcommand\au{\uparrow}
\newcommand\Au{\Uparrow}
\renewcommand\to{\mapsto}

% reduction relations
\newcommand\ab{\a_\b}
\newcommand\ai{\a_\io}
\renewcommand\ae{\a_\eta}
\newcommand\abe{\a_{\b\eta}}
\newcommand\abi{\a_{\b\io}}
\newcommand\abei{\a_{\b\eta\io}}
\newcommand\ar{\a_\cR}
\newcommand\abr{\a_{\b\cR}}
\newcommand\aber{\a_{\b\eta\cR}}

% delimiters
\newcommand\ps[1]{{\langle #1\rangle}}
\newcommand\dps[1]{\ps{\!\ps{#1}\!}}
%\newcommand\I[1]{[\![#1]\!]}
\newcommand\I[1]{\llbracket{#1}\rrbracket}% stmaryrd
\newcommand\J[1]{(\!|#1|\!)}
\newcommand\K[1]{\ps{\!|#1|\!}}

% fonts
\newcommand\bs{\boldsymbol}

% other symbols
\newcommand\ex{\exists}
\newcommand\all{\forall}
\newcommand\ou{\vee}
\newcommand\bigou{\bigvee}
\newcommand\biget{\bigwedge}
\newcommand\et{\wedge}
\newcommand\non{\neg}
%\newcommand\st{\star}
\newcommand\B{\Box}
\renewcommand\th{\vdash}

% orderings
\newcommand\sle{\subseteq}
\newcommand\sge{\supseteq}
\newcommand\slt{\subset}
\newcommand\sgt{\supset}
\newcommand\tle{\unlhd}
\newcommand\tge{\unrhd}
\newcommand\tlt{\lhd}
\newcommand\tgt{\rhd}
\newcommand\cle{\preceq}
\newcommand\cge{\succeq}
\newcommand\clt{\prec}
\newcommand\cgt{\succ}
\newcommand\qle{\sqsubseteq}
\newcommand\qge{\sqsupseteq}
\newcommand\qlt{\sqsubset}
\newcommand\qgt{\sqsupset}

% decorations
\newcommand\h[1]{{\widehat{#1}}}
\renewcommand\o[1]{{\overline{#1}}}
\renewcommand\u[1]{{\underline{#1}}}
\newcommand\q[1]{{\widetilde{#1}}}

% greek letters
\newcommand\al{\alpha}
\renewcommand\b{\beta}
\newcommand\g{\gamma}
\newcommand\G{\Gamma}
\renewcommand\d{\delta}
\newcommand\D{\Delta}
\newcommand\ep{\epsilon}
\newcommand\vep{\varepsilon}
\newcommand\z{\zeta}
\renewcommand\t{\theta}
\newcommand\T{\Theta}
\newcommand\io{\iota}
\newcommand\kap{\kappa}
\renewcommand\l{\lambda}
\renewcommand\L{\Lambda}
\renewcommand\r{\rho}
\newcommand\s{\sigma}
\renewcommand\S{\Sigma}
\newcommand\up{\upsilon}
\newcommand\Up{\Upsilon}
\newcommand\vphi{\varphi}
\newcommand\w{\omega}
\newcommand\W{\Omega}

% math styles
\newcommand\mi{\mathit}
\newcommand\mc{\mathcal}
\newcommand\mt{\mathtt}
\newcommand\mr{\mathrm}
\newcommand\mb{\mathbb}
\newcommand\mg{\mathbf}
\newcommand\mk{\mathfrak}
\newcommand\ms{\mathsf}

% bb upper-case letters
\newcommand\bA{\mb{A}}
\newcommand\bB{\mb{B}}
\newcommand\bC{\mb{C}}
\newcommand\bD{\mb{D}}
\newcommand\bE{\mb{E}}
\newcommand\bF{\mb{F}}
\newcommand\bG{\mb{G}}
\newcommand\bH{\mb{H}}
\newcommand\bI{\mb{I}}
\newcommand\bJ{\mb{J}}
\newcommand\bK{\mb{K}}
\newcommand\bL{\mb{L}}
\newcommand\bM{\mb{M}}
\newcommand\bN{\mb{N}}
\newcommand\bO{\mb{O}}
\newcommand\bP{\mb{P}}
\newcommand\bQ{\mb{Q}}
\newcommand\bR{\mb{R}}
\newcommand\bS{\mb{S}}
\newcommand\bT{\mb{T}}
\newcommand\bU{\mb{U}}
\newcommand\bV{\mb{V}}
\newcommand\bW{\mb{W}}
\newcommand\bX{\mb{X}}
\newcommand\bY{\mb{Y}}
\newcommand\bZ{\mb{Z}}

% calligraphical upper-case letters
\newcommand\cA{\mc{A}}
\newcommand\cB{\mc{B}}
\newcommand\cC{\mc{C}}
\newcommand\cD{\mc{D}}
\newcommand\cE{\mc{E}}
\newcommand\cF{\mc{F}}
\newcommand\cG{\mc{G}}
\newcommand\cH{\mc{H}}
\newcommand\cI{\mc{I}}
\newcommand\cJ{\mc{J}}
\newcommand\cK{\mc{K}}
\newcommand\cL{\mc{L}}
\newcommand\cM{\mc{M}}
\newcommand\cN{\mc{N}}
\newcommand\cO{\mc{O}}
\newcommand\cP{\mc{P}}
\newcommand\cQ{\mc{Q}}
\newcommand\cR{\mc{R}}
\newcommand\cS{\mc{S}}
\newcommand\cT{\mc{T}}
\newcommand\cU{\mc{U}}
\newcommand\cV{\mc{V}}
\newcommand\cW{\mc{W}}
\newcommand\cX{\mc{X}}
\newcommand\cY{\mc{Y}}
\newcommand\cZ{\mc{Z}}

% lower-case frak letters
\newcommand\ka{\mk{a}}
\newcommand\kb{\mk{b}}
\newcommand\kc{\mk{c}}
\newcommand\kd{\mk{d}}
\newcommand\ke{\mk{e}}
\newcommand\kf{\mk{f}}
\newcommand\kg{\mk{g}}
\newcommand\kh{\mk{h}}
\newcommand\ki{\mk{i}}
\newcommand\kj{\mk{j}}
\newcommand\kk{\mk{k}}
\newcommand\kl{\mk{l}}
\newcommand\km{\mk{m}}
\newcommand\kn{\mk{n}}
\newcommand\ko{\mk{o}}
\newcommand\kp{\mk{p}}
\newcommand\kq{\mk{q}}
\newcommand\kr{\mk{r}}
\newcommand\ks{\mk{s}}
\newcommand\kt{\mk{t}}
\newcommand\ku{\mk{u}}
\newcommand\kv{\mk{v}}
\newcommand\kw{\mk{w}}
\newcommand\kx{\mk{x}}
\newcommand\ky{\mk{y}}
\newcommand\kz{\mk{z}}

% upper-case frak letters
\newcommand\kA{\mk{A}}
\newcommand\kB{\mk{B}}
\newcommand\kC{\mk{C}}
\newcommand\kD{\mk{D}}
\newcommand\kE{\mk{E}}
\newcommand\kF{\mk{F}}
\newcommand\kG{\mk{G}}
\newcommand\kH{\mk{H}}
\newcommand\kI{\mk{I}}
\newcommand\kJ{\mk{J}}
\newcommand\kK{\mk{K}}
\newcommand\kL{\mk{L}}
\newcommand\kM{\mk{M}}
\newcommand\kN{\mk{N}}
\newcommand\kO{\mk{O}}
\newcommand\kP{\mk{P}}
\newcommand\kQ{\mk{Q}}
\newcommand\kR{\mk{R}}
\newcommand\kS{\mk{S}}
\newcommand\kT{\mk{T}}
\newcommand\kU{\mk{U}}
\newcommand\kV{\mk{V}}
\newcommand\kW{\mk{W}}
\newcommand\kX{\mk{X}}
\newcommand\kY{\mk{Y}}
\newcommand\kZ{\mk{Z}}

% lower-case sans-serif letters
\newcommand\sa{\ms{a}}
\renewcommand\sb{\ms{b}}
\renewcommand\sc{\ms{c}}
\newcommand\sd{\ms{d}}
\newcommand\se{\ms{e}}
\renewcommand\sf{\ms{f}}
\newcommand\sg{\ms{g}}
\newcommand\sh{\ms{h}}
\newcommand\si{\ms{i}}
\newcommand\sj{\ms{j}}
\newcommand\sk{\ms{k}}
\renewcommand\sl{\ms{l}}
\newcommand\sm{\ms{m}}
\newcommand\sn{\ms{n}}
%\newcommand\so{\ms{o}}
\renewcommand\sp{\ms{p}}
\newcommand\sq{\ms{q}}
\newcommand\sr{\ms{r}}
\renewcommand\ss{\ms{s}}
%\newcommand\st{\ms{t}}
\newcommand\su{\ms{u}}
\newcommand\sv{\ms{v}}
\newcommand\sw{\ms{w}}
\newcommand\sx{\ms{x}}
\newcommand\sy{\ms{y}}
\newcommand\sz{\ms{z}}

% upper-case sans-serif letters
\newcommand\sA{\ms{A}}
\newcommand\sB{\ms{B}}
\newcommand\sC{\ms{C}}
\newcommand\sD{\ms{D}}
\newcommand\sE{\ms{E}}
\newcommand\sF{\ms{F}}
\newcommand\sG{\ms{G}}
\newcommand\sH{\ms{H}}
\newcommand\sI{\ms{I}}
\newcommand\sJ{\ms{J}}
\newcommand\sK{\ms{K}}
\newcommand\sL{\ms{L}}
\newcommand\sM{\ms{M}}
\newcommand\sN{\ms{N}}
\newcommand\sO{\ms{O}}
\newcommand\sP{\ms{P}}
\newcommand\sQ{\ms{Q}}
\newcommand\sR{\ms{R}}
\newcommand\sS{\ms{S}}
\newcommand\sT{\ms{T}}
\newcommand\sU{\ms{U}}
\newcommand\sV{\ms{V}}
\newcommand\sW{\ms{W}}
\newcommand\sX{\ms{X}}
\newcommand\sY{\ms{Y}}
\newcommand\sZ{\ms{Z}}

% lower-case vectors
\newcommand\va{{\vec{a}}}
\newcommand\vb{{\vec{b}}}
\newcommand\vc{{\vec{c}}}
\newcommand\vd{{\vec{d}}}
\newcommand\ve{{\vec{e}}}
\newcommand\vf{{\vec{f}}}
\newcommand\vg{{\vec{g}}}
\newcommand\vh{{\vec{h}}}
\newcommand\vi{{\vec{i}}}
\newcommand\vj{{\vec{j}}}
\newcommand\vk{{\vec{k}}}
\newcommand\vl{{\vec{l}}}
\newcommand\vm{{\vec{m}}}
\newcommand\vn{{\vec{n}}}
\newcommand\vo{{\vec{o}}}
\newcommand\vp{{\vec{p}}}
\newcommand\vq{{\vec{q}}}
\newcommand\vr{{\vec{r}}}
\newcommand\vs{{\vec{s}}}
\newcommand\vt{{\vec{t}}}
\newcommand\vu{{\vec{u}}}
\newcommand\vv{{\vec{v}}}
\newcommand\vw{{\vec{w}}}
\newcommand\vx{{\vec{x}}}
\newcommand\vy{{\vec{y}}}
\newcommand\vz{{\vec{z}}}

% upper-case vectors
\newcommand\vA{{\vec{A}}}
\newcommand\vB{{\vec{B}}}
\newcommand\vC{{\vec{C}}}
\newcommand\vD{{\vec{D}}}
\newcommand\vE{{\vec{E}}}
\newcommand\vF{{\vec{F}}}
\newcommand\vG{{\vec{G}}}
\newcommand\vH{{\vec{H}}}
\newcommand\vI{{\vec{I}}}
\newcommand\vJ{{\vec{J}}}
\newcommand\vK{{\vec{K}}}
\newcommand\vL{{\vec{L}}}
\newcommand\vM{{\vec{M}}}
\newcommand\vN{{\vec{N}}}
\newcommand\vO{{\vec{O}}}
\newcommand\vP{{\vec{P}}}
\newcommand\vQ{{\vec{Q}}}
\newcommand\vR{{\vec{R}}}
\newcommand\vS{{\vec{S}}}
\newcommand\vT{{\vec{T}}}
\newcommand\vU{{\vec{U}}}
\newcommand\vV{{\vec{V}}}
\newcommand\vW{{\vec{W}}}
\newcommand\vX{{\vec{X}}}
\newcommand\vY{{\vec{Y}}}
\newcommand\vZ{{\vec{Z}}}

% appendixes
\newcommand\beginappendixes{\setcounter{section}{0}%
  \renewcommand\thesection{\Alph{section}}}
\newcommand\append[1]{\newpage\refstepcounter{section}%
  \section*{Appendix \thesection: #1}}

% indexes
\newcommand\indlem[2][]{Lem. \ref{#1}}
\newcommand\inddef[2][]{Def. \ref{#1}}
\newcommand\indthm[2][]{Thm. \ref{#1}}
\newcommand\indcor[2][]{Cor. \ref{#1}}
\newcommand\indfig[2][]{Fig. \ref{#1}}
\newcommand\indsec[2][]{Sec. \ref{#1}}
\newcommand\indrem[2][]{Rem. \ref{#1}}
\newcommand\indconj[2][]{Conj. \ref{#1}}
\newcommand\indchap[2][]{Chap. \ref{#1}}
\newcommand\indtxt[2][]{#1}
\newcommand\indpage[1]{page #1}

% environment for rules, etc.
\newenvironment{rul}
  {$\begin{array}{rcl}}
  {\end{array}$}
\newenvironment{rulc}
  {\begin{center}\begin{rul}}
  {\end{rul}\end{center}}

% rule environment
\newenvironment{rew}[1][~~\a~~]
  {$\begin{array}{r@{#1}l}}
  {\end{array}$}
\newenvironment{rewc}[1][~~\a~~]
  {\begin{center}\begin{rew}[#1]}
  {\end{rew}\end{center}}

% rule environment
\newenvironment{typ}[1][\,:\,]{\begin{rew}[#1]}{\end{rew}}
\newenvironment{typc}[1][\,:\,]{\begin{rewc}[#1]}{\end{rewc}}

% theorem-like environments
\newcounter{counter}
\newcounter{dfnnum}
\newcounter{lemnum}
\newcounter{thmnum}
\newcounter{cornum}
\newcounter{remnum}
\newcounter{propnum}
\newcounter{hypnum}
\newcounter{conjnum}
\newcounter{asmnum}
\newcounter{explnum}
{\theorembodyfont{\rmfamily}
  \newtheorem{definition}[dfnnum]{Definition}
  \newtheorem{lemma}[lemnum]{Lemma}
  \newtheorem{theorem}[thmnum]{Theorem}
  \newtheorem{corollary}[cornum]{Corollary}
  \newtheorem{remark}[remnum]{Remark}
  \newtheorem{proposition}[propnum]{Property}
  \newtheorem{conjecture}[conjnum]{Conjecture}
  \newtheorem{hypothesis}[hypnum]{Hypothesis}
  \newtheorem{assumption}[asmnum]{Assumption}
  \newtheorem{example}[explnum]{Example}
}

% proof environment
\newcommand\cqfd{\hfill$\blacksquare$}
\newenvironment{proof}{{\bf Proof.}}{}

% list environment
\leftmargini=4mm
\leftmarginii=3mm
\leftmarginiii=3mm
\leftmarginiv=3mm
\leftmarginv=3mm
\leftmarginvi=3mm

\newenvironment{lstgeneric}[2]
  {\begin{list}{#1}{\topsep=.5mm\itemsep=.5mm\parsep=0mm%
    \itemindent=-3ex\labelsep=1ex\labelwidth=0ex #2}}
  {\end{list}}

\newenvironment{lst}[1]
  {\begin{lstgeneric}{#1}{\itemindent=-1ex}}
  {\end{lstgeneric}}

\newenvironment{enumi}[1]
  {\begin{lstgeneric}{}{\usecounter{enumi}\leftmargin=7mm%
    \renewcommand\makelabel{(#1\arabic{enumi})}}}
  {\end{lstgeneric}}

\newenvironment{bfenumi}[1]
  {\begin{lstgeneric}{}{\usecounter{enumi}\leftmargin=7mm%
    \renewcommand\makelabel{\bf(#1\arabic{enumi})}}}
  {\end{lstgeneric}}

\newenvironment{enumii}[1]
  {\begin{lstgeneric}{}{\usecounter{enumii}%
    \renewcommand\makelabel{(#1\arabic{enumii})}}}
  {\end{lstgeneric}}

\newenvironment{bfenumii}[1]
  {\begin{lstgeneric}{}{\usecounter{enumii}\leftmargin=7mm%
    \renewcommand\makelabel{\bf(#1\arabic{enumii})}}}
  {\end{lstgeneric}}

\newenvironment{enumiii}[1]
  {\begin{lstgeneric}{}{\usecounter{enumiii}%
    \renewcommand\makelabel{(#1\arabic{enumiii})}}}
  {\end{lstgeneric}}

\newenvironment{enumalphai}
  {\begin{lstgeneric}{}{\usecounter{enumi}\leftmargin=7mm%
    \renewcommand\makelabel{(\alph{enumi})}}}
  {\end{lstgeneric}}

\newenvironment{bfenumalphai}
  {\begin{lstgeneric}{}{\usecounter{enumi}\leftmargin=7mm%
    \renewcommand\makelabel{\bf(\alph{enumi})}}}
  {\end{lstgeneric}}

\newenvironment{enumalphaii}
  {\begin{lstgeneric}{}{\usecounter{enumii}\leftmargin=10mm%
    \renewcommand\makelabel{(\alph{enumii})}}}
  {\end{lstgeneric}}

\newenvironment{enumalphaiii}
  {\begin{lstgeneric}{}{\usecounter{enumiii}%
    \renewcommand\makelabel{(\alph{enumiii})}}}
  {\end{lstgeneric}}

% program environment
\newenvironment{prg}
   {\begin{ttfamily}\begin{tabbing}%
      aaa\=aaa\=aaa\=aaa\=aaa\=aaa\=aaa\=\kill}
   {\end{tabbing}\end{ttfamily}}


